LazyFormer: Self Attention with Lazy Update

Improving the efficiency of Transformer-based language pre-training is an important task in NLP, especially for the self-attention module, which is computationally expensive. In this paper, we propose a simple but effective solution, called \emph{LazyFormer}, which computes the self-attention distribution infrequently. LazyFormer composes of multiple lazy blocks, each of which contains multiple Transformer layers. In each lazy block, the self-attention distribution is only computed once in the first layer and then is reused in all upper layers. In this way, the cost of computation could be largely saved. We also provide several training tricks for LazyFormer. Extensive experiments demonstrate the effectiveness of the proposed method.

==> bib_old.tex <==
@article{xiao2019sharing,
  title={Sharing attention weights for fast transformer},
  author={Xiao, Tong and Li, Yinqiao and Zhu, Jingbo and Yu, Zhengtao and Liu, Tongran},
  journal={arXiv preprint arXiv:1906.11024},
  year={2019}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6000--6010},
  year={2017}
}

@article{dai2019transformer,
  title={Transformer-xl: Attentive language models beyond a fixed-length context},
  author={Dai, Zihang and Yang, Zhilin and Yang, Yiming and Carbonell, Jaime and Le, Quoc V and Salakhutdinov, Ruslan},
  journal={arXiv preprint arXiv:1901.02860},
  year={2019}
}

@book{kohler2008quantitative,
  title={Quantitative Linguistik/Quantitative Linguistics: Ein internationales Handbuch/An International Handbook},
  author={K{\"o}hler, Reinhard and Altmann, Gabriel and Piotrowski, Rajmund G},
  volume={27},
  year={2008},
  publisher={Walter de Gruyter}
}

@article{snell2019word,
  title={Word position coding in reading is noisy},
  author={Snell, Joshua and Grainger, Jonathan},
  journal={Psychonomic bulletin \& review},
  volume={26},
  number={2},
  pages={609--615},
  year={2019},
  publisher={Springer}
}

@inproceedings{mikolov2013distributed,
  title={Distributed representations of words and phrases and their compositionality},
  author={Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
  booktitle={Advances in neural information processing systems},
  pages={3111--3119},
  year={2013}
}

@book{gray2006toeplitz,
  title={Toeplitz and circulant matrices: A review},
  author={Gray, Robert M},
  year={2006},
  publisher={now publishers inc}
}

@article{xiong2020layer,
  title={On layer normalization in the transformer architecture},
  author={Xiong, Ruibin and Yang, Yunchang and He, Di and Zheng, Kai and Zheng, Shuxin and Xing, Chen and Zhang, Huishuai and Lan, Yanyan and Wang, Liwei and Liu, Tie-Yan},
  journal={arXiv preprint arXiv:2002.04745},
  year={2020}
}

% @inproceedings{liu2019mt-dnn,
%     title = "Multi-Task Deep Neural Networks for Natural Language Understanding",
%     author = "Liu, Xiaodong and He, Pengcheng and Chen, Weizhu and Gao, Jianfeng",
%     booktitle = "Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics",
%     month = jul,
%     year = "2019",
%     address = "Florence, Italy",
%     publisher = "Association for Computational Linguistics",
%     url = "https://www.aclweb.org/anthology/P19-1441",
%     pages = "4487--4496"
% }

@article{warstadt2018neural,
    title={Neural Network Acceptability Judgments},
    author={Warstadt, Alex and Singh, Amanpreet and Bowman, Samuel R},
    journal={arXiv preprint arXiv:1805.12471},
    year={2018}
}

@article{ott2019fairseq,
  title={fairseq: A fast, extensible toolkit for sequence modeling},
  author={Ott, Myle and Edunov, Sergey and Baevski, Alexei and Fan, Angela and Gross, Sam and Ng, Nathan and Grangier, David and Auli, Michael},
  journal={arXiv preprint arXiv:1904.01038},
  year={2019}
}

@article{strubell2019energy,
  title={Energy and Policy Considerations for Deep Learning in NLP},
  author={Strubell, Emma and Ganesh, Ananya and McCallum, Andrew},
  journal={arXiv preprint arXiv:1906.02243},
  year={2019}
}

@article{liu2019multi,
  title={Multi-task deep neural networks for natural language understanding},
  author={Liu, Xiaodong and He, Pengcheng and Chen, Weizhu and Gao, Jianfeng},
  journal={arXiv preprint arXiv:1901.11504},
  year={2019}
}

@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle={Advances in neural information processing systems},
  pages={2672--2680},
  year={2014}
}

@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
  journal={arXiv preprint arXiv:1503.02531},
  year={2015}
} 
@inproceedings{bengio2009curriculum,
  title={Curriculum learning},
  author={Bengio, Yoshua and Louradour, J{\'e}r{\^o}me and Collobert, Ronan and Weston, Jason},
  booktitle={Proceedings of the 26th annual international conference on machine learning},
  pages={41--48},
  year={2009}
}

@article{ambrus2017case,
  title={The case for nil votes: Voter behavior under asymmetric information in compulsory and voluntary voting systems},
  author={Ambrus, Attila and Greiner, Ben and Sastro, Anne},
  journal={Journal of Public Economics},
  volume={154},
  pages={34--48},
  year={2017},
  publisher={Elsevier}
}

@article{feddersen1999abstention,
  title={Abstention in elections with asymmetric information and diverse preferences},
  author={Feddersen, Timothy J and Pesendorfer, Wolfgang},
  journal={American Political Science Review},
  volume={93},
  number={2},
  pages={381--398},
  year={1999},
  publisher={Cambridge University Press}
}

@inproceedings{dong2019unified,
  title={Unified language model pre-training for natural language understanding and generation},
  author={Dong, Li and Yang, Nan and Wang, Wenhui and Wei, Furu and Liu, Xiaodong and Wang, Yu and Gao, Jianfeng and Zhou, Ming and Hon, Hsiao-Wuen},
  booktitle={Advances in Neural Information Processing Systems},
  pages={13042--13054},
  year={2019}
}

@inproceedings{gong2019efficient,
  title={Efficient training of bert by progressively stacking},
  author={Gong, Linyuan and He, Di and Li, Zhuohan and Qin, Tao and Wang, Liwei and Liu, Tieyan},
  booktitle={International Conference on Machine Learning},
  pages={2337--2346},
  year={2019}
}

@article{hochreiter1997long,
	title={Long short-term memory},
	author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
	journal={Neural computation},
	volume={9},
	number={8},
	pages={1735--1780},
	year={1997},
	publisher={MIT Press}
}

@article{you2019large,
  title={Large batch optimization for deep learning: Training bert in 76 minutes},
  author={You, Yang and Li, Jing and Reddi, Sashank and Hseu, Jonathan and Kumar, Sanjiv and Bhojanapalli, Srinadh and Song, Xiaodan and Demmel, James and Hsieh, Cho-Jui},
  journal={arXiv preprint arXiv:1904.00962},
  volume={1},
  number={5},
  year={2019}
}

@inproceedings{clark2019electra,
  title={ELECTRA: Pre-training Text Encoders as Discriminators Rather Than Generators},
  author={Clark, Kevin and Luong, Minh-Thang and Le, Quoc V and Manning, Christopher D},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}


@inproceedings{sutskever2014sequence,
  title={Sequence to sequence learning with neural networks},
  author={Sutskever, Ilya and Vinyals, Oriol and Le, Quoc V},
  booktitle={Advances in neural information processing systems},
  pages={3104--3112},
  year={2014}
}

@article{radford2019language,
  title={Language models are unsupervised multitask learners},
  author={Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya},
  journal={OpenAI Blog},
  volume={1},
  number={8},
  year={2019}
}

@article{joulin2016fasttext,
  title={Fasttext. zip: Compressing text classification models},
  author={Joulin, Armand and Grave, Edouard and Bojanowski, Piotr and Douze, Matthijs and J{\'e}gou, H{\'e}rve and Mikolov, Tomas},
  journal={arXiv preprint arXiv:1612.03651},
  year={2016}
}

@inproceedings{pennington2014glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher D},
  booktitle={Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP)},
  pages={1532--1543},
  year={2014}
}

@article{yang2019xlnet,
  title={XLNet: Generalized Autoregressive Pretraining for Language Understanding},
  author={Yang, Zhilin and Dai, Zihang and Yang, Yiming and Carbonell, Jaime and Salakhutdinov, Ruslan and Le, Quoc V},
  journal={arXiv preprint arXiv:1906.08237},
  year={2019}
}


@article{liu2019roberta,
  title={Roberta: A robustly optimized bert pretraining approach},
  author={Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
  journal={arXiv preprint arXiv:1907.11692},
  year={2019}
}

@article{hinton2012deep,
  title={Deep neural networks for acoustic modeling in speech recognition: The shared views of four research groups},
  author={Hinton, Geoffrey and Deng, Li and Yu, Dong and Dahl, George E and Mohamed, Abdel-rahman and Jaitly, Navdeep and Senior, Andrew and Vanhoucke, Vincent and Nguyen, Patrick and Sainath, Tara N and others},
  journal={IEEE Signal processing magazine},
  volume={29},
  number={6},
  pages={82--97},
  year={2012},
  publisher={IEEE}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={Computer Vision and Pattern Recognition, 2009. CVPR 2009. IEEE Conference on},
  pages={248--255},
  year={2009},
  organization={Ieee}
}

@inproceedings{socher2011dynamic,
  title={Dynamic pooling and unfolding recursive autoencoders for paraphrase detection},
  author={Socher, Richard and Huang, Eric H and Pennin, Jeffrey and Manning, Christopher D and Ng, Andrew Y},
  booktitle={Advances in neural information processing systems},
  pages={801--809},
  year={2011}
}

@article{tai2015improved,
  title={Improved semantic representations from tree-structured long short-term memory networks},
  author={Tai, Kai Sheng and Socher, Richard and Manning, Christopher D},
  journal={arXiv preprint arXiv:1503.00075},
  year={2015}
}

@article{kalchbrenner2014convolutional,
  title={A convolutional neural network for modelling sentences},
  author={Kalchbrenner, Nal and Grefenstette, Edward and Blunsom, Phil},
  journal={arXiv preprint arXiv:1404.2188},
  year={2014}
}

@article{peters2018deep,
  title={Deep contextualized word representations},
  author={Peters, Matthew E and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  journal={arXiv preprint arXiv:1802.05365},
  year={2018}
}

% @article{radford2018improving,
%   title={Improving language understanding by generative pre-training},
%   author={Radford, Alec and Narasimhan, Karthik and Salimans, Tim and Sutskever, Ilya},
%   journal={URL https://s3-us-west-2. amazonaws. com/openai-assets/research-covers/language-unsupervised/language\_ understanding\_paper. pdf},
%   year={2018}
% }

@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@article{dehghani2018universal,
  title={Universal transformers},
  author={Dehghani, Mostafa and Gouws, Stephan and Vinyals, Oriol and Uszkoreit, Jakob and Kaiser, {\L}ukasz},
  journal={arXiv preprint arXiv:1807.03819},
  year={2018}
}

@article{chen2015net2net,
  title={Net2net: Accelerating learning via knowledge transfer},
  author={Chen, Tianqi and Goodfellow, Ian and Shlens, Jonathon},
  journal={arXiv preprint arXiv:1511.05641},
  year={2015}
}

@inproceedings{gehring2017convs2s,
  author    = {Gehring, Jonas, and Auli, Michael and Grangier, David and Yarats, Denis and Dauphin, Yann N},
  title     = "{Convolutional Sequence to Sequence Learning}",
  booktitle = {Proc. of International Conference on Machine Learning},
  year      = 2017,
}

@inproceedings{moviebook,
title = {Aligning Books and Movies: Towards Story-like Visual Explanations by Watching Movies and Reading Books},
author = {Yukun Zhu and Ryan Kiros and Richard Zemel and Ruslan Salakhutdinov and Raquel Urtasun and Antonio Torralba and Sanja Fidler},
booktitle = {arXiv preprint arXiv:1506.06724},
year = {2015}
}

@inproceedings{Koehn2007MosesOS,
  title={Moses: Open Source Toolkit for Statistical Machine Translation},
  author={Philipp Koehn and Hieu Hoang and Alexandra Birch and Chris Callison-Burch and Marcello Federico and Nicola Bertoldi and Brooke Cowan and Wade Shen and Christine Moran and Richard Zens and Chris Dyer and Ondrej Bojar and Alexandra Constantin and Evan Herbst},
  booktitle={ACL},
  year={2007}
}

% @article{DBLP:journals/corr/SennrichHB15,
%   author    = {Rico Sennrich and
%               Barry Haddow and
%               Alexandra Birch},
%   title     = {Neural Machine Translation of Rare Words with Subword Units},
%   journal   = {CoRR},
%   volume    = {abs/1508.07909},
%   year      = {2015},
%   url       = {http://arxiv.org/abs/1508.07909},
%   archivePrefix = {arXiv},
%   eprint    = {1508.07909},
%   timestamp = {Mon, 13 Aug 2018 16:47:17 +0200},
%   biburl    = {https://dblp.org/rec/bib/journals/corr/SennrichHB15},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
% }

% @article{DBLP:journals/corr/abs-1804-07461,
%   author    = {Alex Wang and
%               Amanpreet Singh and
%               Julian Michael and
%               Felix Hill and
%               Omer Levy and
%               Samuel R. Bowman},
%   title     = {{GLUE:} {A} Multi-Task Benchmark and Analysis Platform for Natural
%               Language Understanding},
%   journal   = {CoRR},
%   volume    = {abs/1804.07461},
%   year      = {2018},
%   url       = {http://arxiv.org/abs/1804.07461},
%   archivePrefix = {arXiv},
%   eprint    = {1804.07461},
%   timestamp = {Mon, 13 Aug 2018 16:46:56 +0200},
%   biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1804-07461},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
% }

% @article{DBLP:journals/corr/KingmaB14,
%   author    = {Diederik P. Kingma and
%               Jimmy Ba},
%   title     = {Adam: {A} Method for Stochastic Optimization},
%   journal   = {CoRR},
%   volume    = {abs/1412.6980},
%   year      = {2014},
%   url       = {http://arxiv.org/abs/1412.6980},
%   archivePrefix = {arXiv},
%   eprint    = {1412.6980},
%   timestamp = {Mon, 13 Aug 2018 16:47:35 +0200},
%   biburl    = {https://dblp.org/rec/bib/journals/corr/KingmaB14},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
% }

@article{micikevicius2017mixed,
  title={Mixed precision training},
  author={Micikevicius, Paulius and Narang, Sharan and Alben, Jonah and Diamos, Gregory and Elsen, Erich and Garcia, David and Ginsburg, Boris and Houston, Michael and Kuchaiev, Oleksii and Venkatesh, Ganesh and others},
  journal={arXiv preprint arXiv:1710.03740},
  year={2017}
}

% @article{DBLP:journals/corr/HeZRS15,
%   author    = {Kaiming He and
%               Xiangyu Zhang and
%               Shaoqing Ren and
%               Jian Sun},
%   title     = {Deep Residual Learning for Image Recognition},
%   journal   = {CoRR},
%   volume    = {abs/1512.03385},
%   year      = {2015},
%   url       = {http://arxiv.org/abs/1512.03385},
%   archivePrefix = {arXiv},
%   eprint    = {1512.03385},
%   timestamp = {Mon, 13 Aug 2018 16:46:56 +0200},
%   biburl    = {https://dblp.org/rec/bib/journals/corr/HeZRS15},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
% }

% @article{DBLP:journals/corr/BahdanauCB14,
%   author    = {Dzmitry Bahdanau and
%               Kyunghyun Cho and
%               Yoshua Bengio},
%   title     = {Neural Machine Translation by Jointly Learning to Align and Translate},
%   journal   = {CoRR},
%   volume    = {abs/1409.0473},
%   year      = {2014},
%   url       = {http://arxiv.org/abs/1409.0473},
%   archivePrefix = {arXiv},
%   eprint    = {1409.0473},
%   timestamp = {Mon, 13 Aug 2018 16:46:05 +0200},
%   biburl    = {https://dblp.org/rec/bib/journals/corr/BahdanauCB14},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
% }

@article{hendrycks2016gaussian,
  title={Gaussian error linear units (gelus)},
  author={Hendrycks, Dan and Gimpel, Kevin},
  journal={arXiv preprint arXiv:1606.08415},
  year={2016}
}

@article{paszke2017automatic,
  title={Automatic differentiation in pytorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  year={2017}
}

@book{lass2014speech,
  title={Speech and language: advances in basic research and practice},
  author={Lass, Norman J},
  year={2014},
  publisher={Academic Press}
}

@article{ba2016layer,
  title={Layer normalization},
  author={Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E},
  journal={arXiv preprint arXiv:1607.06450},
  year={2016}
}

@article{he2020deberta,
  title={DeBERTa: Decoding-enhanced BERT with Disentangled Attention},
  author={He, Pengcheng and Liu, Xiaodong and Gao, Jianfeng and Chen, Weizhu},
  journal={arXiv preprint arXiv:2006.03654},
  year={2020}
}

@article{wang2019encoding,
  title={Encoding word order in complex embeddings},
  author={Wang, Benyou and Zhao, Donghao and Lioma, Christina and Li, Qiuchi and Zhang, Peng and Simonsen, Jakob Grue},
  journal={arXiv preprint arXiv:1912.12333},
  year={2019}
}

@article{liu2020learning,
  title={Learning to Encode Position for Transformer with Continuous Dynamical Model},
  author={Liu, Xuanqing and Yu, Hsiang-Fu and Dhillon, Inderjit and Hsieh, Cho-Jui},
  journal={arXiv preprint arXiv:2003.09229},
  year={2020}
}

@inproceedings{shiv2019novel,
  title={Novel positional encodings to enable tree-based transformers},
  author={Shiv, Vighnesh and Quirk, Chris},
  booktitle={Advances in Neural Information Processing Systems},
  pages={12058--12068},
  year={2019}
}

@article{gehring2017convolutional,
  title={Convolutional sequence to sequence learning},
  author={Gehring, Jonas and Auli, Michael and Grangier, David and Yarats, Denis and Dauphin, Yann N},
  journal={arXiv preprint arXiv:1705.03122},
  year={2017}
}

@article{al2018character,
  title={Character-level language modeling with deeper self-attention},
  author={Al-Rfou, Rami and Choe, Dokook and Constant, Noah and Guo, Mandy and Jones, Llion},
  journal={arXiv preprint arXiv:1808.04444},
  year={2018}
}

@article{bao2020unilmv2,
  title={Unilmv2: Pseudo-masked language models for unified language model pre-training},
  author={Bao, Hangbo and Dong, Li and Wei, Furu and Wang, Wenhui and Yang, Nan and Liu, Xiaodong and Wang, Yu and Piao, Songhao and Gao, Jianfeng and Zhou, Ming and others},
  journal={arXiv preprint arXiv:2002.12804},
  year={2020}
}

@article{edunov2018understanding,
  title={Understanding back-translation at scale},
  author={Edunov, Sergey and Ott, Myle and Auli, Michael and Grangier, David},
  journal={arXiv preprint arXiv:1808.09381},
  year={2018}
}

@article{dehghani2018universal,
  title={Universal transformers},
  author={Dehghani, Mostafa and Gouws, Stephan and Vinyals, Oriol and Uszkoreit, Jakob and Kaiser, {\L}ukasz},
  journal={arXiv preprint arXiv:1807.03819},
  year={2018}
}

@article{clark2019does,
  title={What does BERT look at? An Analysis of BERT’s Attention},
  author={Clark, Kevin and Khandelwal, Urvashi and Levy, Omer and Manning, Christopher D},
  journal={ACL 2019},
  pages={276},
  year={2019}
}

@inproceedings{bengio2009curriculum,
  title={Curriculum learning},
  author={Bengio, Yoshua and Louradour, J{\'e}r{\^o}me and Collobert, Ronan and Weston, Jason},
  booktitle={Proceedings of the 26th annual international conference on machine learning},
  pages={41--48},
  year={2009},
  organization={ACM}
}

@inproceedings{pentina2015curriculum,
  title={Curriculum learning of multiple tasks},
  author={Pentina, Anastasia and Sharmanska, Viktoriia and Lampert, Christoph H},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5492--5500},
  year={2015}
}

@book{vapnik2013nature,
  title={The nature of statistical learning theory},
  author={Vapnik, Vladimir},
  year={2013},
  publisher={Springer science \& business media}
}

@article{van2017dynamic,
  title={Dynamic data selection for neural machine translation},
  author={van der Wees, Marlies and Bisazza, Arianna and Monz, Christof},
  journal={arXiv preprint arXiv:1708.00712},
  year={2017}
}

@article{edunov2017classical,
  title={Classical Structured Prediction Losses for Sequence to Sequence Learning},
  author={Edunov, Sergey and Ott, Myle and Auli, Michael and Grangier, David and Ranzato, Marc'Aurelio},
  journal={arXiv preprint arXiv:1711.04956},
  year={2017}
}

@article{cho2014learning,
  title={Learning phrase representations using RNN encoder-decoder for statistical machine translation},
  author={Cho, Kyunghyun and Van Merri{\"e}nboer, Bart and Gulcehre, Caglar and Bahdanau, Dzmitry and Bougares, Fethi and Schwenk, Holger and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.1078},
  year={2014}
}

@article{bahdanau2014neural,
  title={Neural machine translation by jointly learning to align and translate},
  author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1409.0473},
  year={2014}
}

@article{shen2015minimum,
  title={Minimum risk training for neural machine translation},
  author={Shen, Shiqi and Cheng, Yong and He, Zhongjun and He, Wei and Wu, Hua and Sun, Maosong and Liu, Yang},
  journal={arXiv preprint arXiv:1512.02433},
  year={2015}
}

@article{shen2016neural,
  title={Neural Headline Generation with Sentence-wise Optimization},
  author={Shen, Shiqi and Zhao, Yu and Liu, Zhiyuan and Sun, Maosong and others},
  journal={arXiv preprint arXiv:1604.01904},
  year={2016}
}

@inproceedings{suzuki2017cutting,
  title={Cutting-off Redundant Repeating Generations for Neural Abstractive Summarization},
  author={Suzuki, Jun and Nagata, Masaaki},
  booktitle={Proceedings of the 15th Conference of the European Chapter of the Association for Computational Linguistics: Volume 2, Short Papers},
  volume={2},
  pages={291--297},
  year={2017}
}

@article{wiseman2016sequence,
  title={Sequence-to-sequence learning as beam-search optimization},
  author={Wiseman, Sam and Rush, Alexander M},
  journal={arXiv preprint arXiv:1606.02960},
  year={2016}
}

@article{bahdanau2016actor,
  title={An actor-critic algorithm for sequence prediction},
  author={Bahdanau, Dzmitry and Brakel, Philemon and Xu, Kelvin and Goyal, Anirudh and Lowe, Ryan and Pineau, Joelle and Courville, Aaron and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1607.07086},
  year={2016}
}

@article{huang2017neural,
  title={Neural phrase-based machine translation},
  author={Huang, Po-Sen and Wang, Chong and Zhou, Dengyong and Deng, Li},
  journal={arXiv preprint arXiv:1706.05565},
  year={2017}
}

@article{kalchbrenner2016neural,
  title={Neural machine translation in linear time},
  author={Kalchbrenner, Nal and Espeholt, Lasse and Simonyan, Karen and Oord, Aaron van den and Graves, Alex and Kavukcuoglu, Koray},
  journal={arXiv preprint arXiv:1610.10099},
  year={2016}
}

@article{wu2016google,
  title={Google's neural machine translation system: Bridging the gap between human and machine translation},
  author={Wu, Yonghui and Schuster, Mike and Chen, Zhifeng and Le, Quoc V and Norouzi, Mohammad and Macherey, Wolfgang and Krikun, Maxim and Cao, Yuan and Gao, Qin and Macherey, Klaus and others},
  journal={arXiv preprint arXiv:1609.08144},
  year={2016}
}

@article{eriguchi2016tree,
  title={Tree-to-sequence attentional neural machine translation},
  author={Eriguchi, Akiko and Hashimoto, Kazuma and Tsuruoka, Yoshimasa},
  journal={arXiv preprint arXiv:1603.06075},
  year={2016}
}

@inproceedings{wang2017neural,
  title={Neural Machine Translation Advised by Statistical Machine Translation.},
  author={Wang, Xing and Lu, Zhengdong and Tu, Zhaopeng and Li, Hang and Xiong, Deyi and Zhang, Min},
  booktitle={AAAI},
  pages={3330--3336},
  year={2017}
}

@article{luong2015effective,
  title={Effective approaches to attention-based neural machine translation},
  author={Luong, Minh-Thang and Pham, Hieu and Manning, Christopher D},
  journal={arXiv preprint arXiv:1508.04025},
  year={2015}
}

@article{shazeer2017outrageously,
  title={Outrageously large neural networks: The sparsely-gated mixture-of-experts layer},
  author={Shazeer, Noam and Mirhoseini, Azalia and Maziarz, Krzysztof and Davis, Andy and Le, Quoc and Hinton, Geoffrey and Dean, Jeff},
  journal={arXiv preprint arXiv:1701.06538},
  year={2017}
}

@article{rush2015neural,
  title={A neural attention model for abstractive sentence summarization},
  author={Rush, Alexander M and Chopra, Sumit and Weston, Jason},
  journal={arXiv preprint arXiv:1509.00685},
  year={2015}
}

@inproceedings{serban2016building,
  title={Building End-To-End Dialogue Systems Using Generative Hierarchical Neural Network Models.},
  author={Serban, Iulian Vlad and Sordoni, Alessandro and Bengio, Yoshua and Courville, Aaron C and Pineau, Joelle},
  booktitle={AAAI},
  volume={16},
  pages={3776--3784},
  year={2016}
}

@article{vijayakumar2016diverse,
  title={Diverse beam search: Decoding diverse solutions from neural sequence models},
  author={Vijayakumar, Ashwin K and Cogswell, Michael and Selvaraju, Ramprasath R and Sun, Qing and Lee, Stefan and Crandall, David and Batra, Dhruv},
  journal={arXiv preprint arXiv:1610.02424},
  year={2016}
}

@article{sennrich2015neural,
  title={Neural machine translation of rare words with subword units},
  author={Sennrich, Rico and Haddow, Barry and Birch, Alexandra},
  journal={arXiv preprint arXiv:1508.07909},
  year={2015}
}

@article{gehring2016convolutional,
  title={A convolutional encoder model for neural machine translation},
  author={Gehring, Jonas and Auli, Michael and Grangier, David and Dauphin, Yann N},
  journal={arXiv preprint arXiv:1611.02344},
  year={2016}
}

@inproceedings{chung2015gated,
  title={Gated feedback recurrent neural networks},
  author={Chung, Junyoung and Gulcehre, Caglar and Cho, Kyunghyun and Bengio, Yoshua},
  booktitle={International Conference on Machine Learning},
  pages={2067--2075},
  year={2015}
}

@inproceedings{koehn2004pharaoh,
  title={Pharaoh: a beam search decoder for phrase-based statistical machine translation models},
  author={Koehn, Philipp},
  booktitle={Conference of the Association for Machine Translation in the Americas},
  pages={115--124},
  year={2004},
  organization={Springer}
}

@inproceedings{germann2003greedy,
  title={Greedy decoding for statistical machine translation in almost linear time},
  author={Germann, Ulrich},
  booktitle={Proceedings of the 2003 Conference of the North American Chapter of the Association for Computational Linguistics on Human Language Technology-Volume 1},
  pages={1--8},
  year={2003},
  organization={Association for Computational Linguistics}
}

@inproceedings{cettolo2014report,
  title={Report on the 11th IWSLT evaluation campaign, IWSLT 2014},
  author={Cettolo, Mauro and Niehues, Jan and St{\"u}ker, Sebastian and Bentivogli, Luisa and Federico, Marcello},
  booktitle={Proceedings of the International Workshop on Spoken Language Translation, Hanoi, Vietnam},
  year={2014}
}

@article{graff2003english,
  title={English gigaword},
  author={Graff, David and Kong, Junbo and Chen, Ke and Maeda, Kazuaki},
  journal={Linguistic Data Consortium, Philadelphia},
  volume={4},
  pages={1},
  year={2003}
}

@article{gibberd2017regularized,
  title={Regularized Estimation of Piecewise Constant Gaussian Graphical Models: The Group-Fused Graphical Lasso},
  author={Gibberd, Alexander J and Nelson, James DB},
  journal={Journal of Computational and Graphical Statistics},
  volume={26},
  number={3},
  pages={623--634},
  year={2017},
  publisher={Taylor \& Francis}
}

@inproceedings{liu2010efficient,
  title={An efficient algorithm for a class of fused lasso problems},
  author={Liu, Jun and Yuan, Lei and Ye, Jieping},
  booktitle={Proceedings of the 16th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={323--332},
  year={2010},
  organization={ACM}
}

@inproceedings{tan2017xmu,
  title={XMU neural machine translation systems for WMT 17},
  author={Tan, Zhixing and Wang, Boli and Hu, Jinming and Chen, Yidong and Shi, Xiaodong},
  booktitle={Proceedings of the Second Conference on Machine Translation},
  pages={400--404},
  year={2017}
}

@article{sennrich2017university,
  title={The University of Edinburgh's Neural MT Systems for WMT17},
  author={Sennrich, Rico and Birch, Alexandra and Currey, Anna and Germann, Ulrich and Haddow, Barry and Heafield, Kenneth and Barone, Antonio Valerio Miceli and Williams, Philip},
  journal={arXiv preprint arXiv:1708.00726},
  year={2017}
}

@inproceedings{wang2017sogou,
  title={Sogou Neural Machine Translation Systems for WMT17},
  author={Wang, Yuguang and Cheng, Shanbo and Jiang, Liyang and Yang, Jiajun and Chen, Wei and Li, Muze and Shi, Lin and Wang, Yanfeng and Yang, Hongtao},
  booktitle={Proceedings of the Second Conference on Machine Translation},
  pages={410--415},
  year={2017}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{graves2005framewise,
  title={Framewise phoneme classification with bidirectional LSTM and other neural network architectures},
  author={Graves, Alex and Schmidhuber, J{\"u}rgen},
  journal={Neural Networks},
  volume={18},
  number={5-6},
  pages={602--610},
  year={2005},
  publisher={Elsevier}
}

@article{zhou2016deep,
  title={Deep recurrent models with fast-forward connections for neural machine translation},
  author={Zhou, Jie and Cao, Ying and Wang, Xuguang and Li, Peng and Xu, Wei},
  journal={arXiv preprint arXiv:1606.04199},
  year={2016}
}

% @article{DBLP:journals/corr/RanzatoCAZ15,
%   author    = {Marc'Aurelio Ranzato and
%               Sumit Chopra and
%               Michael Auli and
%               Wojciech Zaremba},
%   title     = {Sequence Level Training with Recurrent Neural Networks},
%   journal   = {CoRR},
%   volume    = {abs/1511.06732},
%   year      = {2015},
%   url       = {http://arxiv.org/abs/1511.06732},
%   archivePrefix = {arXiv},
%   eprint    = {1511.06732},
%   timestamp = {Wed, 07 Jun 2017 14:41:00 +0200},
%   biburl    = {http://dblp.org/rec/bib/journals/corr/RanzatoCAZ15},
%   bibsource = {dblp computer science bibliography, http://dblp.org}
% }

@article{ranzato2015sequence,
  title={Sequence level training with recurrent neural networks},
  author={Ranzato, Marc'Aurelio and Chopra, Sumit and Auli, Michael and Zaremba, Wojciech},
  journal={arXiv preprint arXiv:1511.06732},
  year={2015}
}

% @inproceedings{DBLP:conf/acl/PapineniRWZ02,
%   author    = {Kishore Papineni and
%               Salim Roukos and
%               Todd Ward and
%               Wei{-}Jing Zhu},
%   title     = {Bleu: a Method for Automatic Evaluation of Machine Translation},
%   booktitle = {Proceedings of the 40th Annual Meeting of the Association for Computational
%               Linguistics, July 6-12, 2002, Philadelphia, PA, {USA.}},
%   pages     = {311--318},
%   year      = {2002},
%   crossref  = {DBLP:conf/acl/2002},
%   url       = {http://www.aclweb.org/anthology/P02-1040.pdf},
%   timestamp = {Thu, 17 Aug 2017 17:55:42 +0200},
%   biburl    = {http://dblp.org/rec/bib/conf/acl/PapineniRWZ02},
%   bibsource = {dblp computer science bibliography, http://dblp.org}
% }

@inproceedings{papineni2002bleu,
  title={BLEU: a method for automatic evaluation of machine translation},
  author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
  booktitle={Proceedings of the 40th annual meeting on association for computational linguistics},
  pages={311--318},
  year={2002},
  organization={Association for Computational Linguistics}
}

@inproceedings{ROUGE,
  title={Rouge: A package for automatic evaluation of summaries},
  author={Lin, Chin-Yew},
  booktitle={ACL-04 workshop},
  year={2004},
  organization={Barcelona, Spain}
}

@article{lin2017focal,
  title={Focal loss for dense object detection},
  author={Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
  journal={arXiv preprint arXiv:1708.02002},
  year={2017}
}

% @inproceedings{DBLP:conf/iccv/LinGGHD17,
%   author    = {Tsung{-}Yi Lin and
%               Priya Goyal and
%               Ross B. Girshick and
%               Kaiming He and
%               Piotr Doll{\'{a}}r},
%   title     = {Focal Loss for Dense Object Detection},
%   booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
%               Italy, October 22-29, 2017},
%   pages     = {2999--3007},
%   year      = {2017},
%   crossref  = {DBLP:conf/iccv/2017},
%   url       = {https://doi.org/10.1109/ICCV.2017.324},
%   doi       = {10.1109/ICCV.2017.324},
%   timestamp = {Thu, 11 Jan 2018 13:21:37 +0100},
%   biburl    = {http://dblp.org/rec/bib/conf/iccv/LinGGHD17},
%   bibsource = {dblp computer science bibliography, http://dblp.org}
% }

@article{lee2016fully,
  title={Fully character-level neural machine translation without explicit segmentation},
  author={Lee, Jason and Cho, Kyunghyun and Hofmann, Thomas},
  journal={arXiv preprint arXiv:1610.03017},
  year={2016}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@article{luong2016achieving,
  title={Achieving open vocabulary neural machine translation with hybrid word-character models},
  author={Luong, Minh-Thang and Manning, Christopher D},
  journal={arXiv preprint arXiv:1604.00788},
  year={2016}
}

@article{belinkov2017neural,
  title={What do Neural Machine Translation Models Learn about Morphology?},
  author={Belinkov, Yonatan and Durrani, Nadir and Dalvi, Fahim and Sajjad, Hassan and Glass, James},
  journal={arXiv preprint arXiv:1704.03471},
  year={2017}
}

@article{He2017Decoding,
  title={Decoding with Value Networks for Neural Machine Translation},
  author={He, Di and Lu, Hanqing and Xia, Yingce and Qin, Tao and Wang, Liwei and Liu, Tieyan},
  booktitle={NIPS},
  year={2017},
}

@inproceedings{kim2016character,
  title={Character-Aware Neural Language Models.},
  author={Kim, Yoon and Jernite, Yacine and Sontag, David and Rush, Alexander M},
  booktitle={AAAI},
  pages={2741--2749},
  year={2016}
}


@article{Kocmi2017Curriculum,
  title={Curriculum Learning and Minibatch Bucketing in Neural Machine Translation},
  journal={arXiv preprint arXiv:1707.09533},
  author={Kocmi, Tom and Bojar, Ondrej},
  year={2017},
}

@article{Szegedy2015Rethinking,
  title={Rethinking the Inception Architecture for Computer Vision},
  journal={arXiv preprint arXiv:1512.00567},
  author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jonathon and Wojna, Zbigniew},
  pages={2818-2826},
  year={2015},
}
@inproceedings{Wang2018Dual,
  title={Dual Transfer Learning for Neural Machine Translation with Marginal Distribution Regularization},
  author={Wang, Yijun and Xia, Yingce and Zhao, Li and Bian, Jiang and Qin, Tao and Liu, Guiquan, and Liu},
  booktitle={AAAI},
  year={2018}
}
@article{shaw2018self,
  title={Self-attention with relative position representations},
  author={Shaw, Peter and Uszkoreit, Jakob and Vaswani, Ashish},
  journal={arXiv preprint arXiv:1803.02155},
  year={2018}
}

@article{raffel2019exploring,
  title={Exploring the limits of transfer learning with a unified text-to-text transformer},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J},
  journal={arXiv preprint arXiv:1910.10683},
  year={2019}
}

@article{wang2020linformer,
  title={Linformer: Self-Attention with Linear Complexity},
  author={Wang, Sinong and Li, Belinda and Khabsa, Madian and Fang, Han and Ma, Hao},
  journal={arXiv preprint arXiv:2006.04768},
  year={2020}
}

@article{beltagy2020longformer,
  title={Longformer: The long-document transformer},
  author={Beltagy, Iz and Peters, Matthew E and Cohan, Arman},
  journal={arXiv preprint arXiv:2004.05150},
  year={2020}
}

@article{lan2019albert,
  title={Albert: A lite bert for self-supervised learning of language representations},
  author={Lan, Zhenzhong and Chen, Mingda and Goodman, Sebastian and Gimpel, Kevin and Sharma, Piyush and Soricut, Radu},
  journal={arXiv preprint arXiv:1909.11942},
  year={2019}
}

@article{zaheer2020big,
  title={Big bird: Transformers for longer sequences},
  author={Zaheer, Manzil and Guruganesh, Guru and Dubey, Kumar Avinava and Ainslie, Joshua and Alberti, Chris and Ontanon, Santiago and Pham, Philip and Ravula, Anirudh and Wang, Qifan and Yang, Li and others},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}

@article{kitaev2020reformer,
  title={Reformer: The efficient transformer},
  author={Kitaev, Nikita and Kaiser, {\L}ukasz and Levskaya, Anselm},
  journal={arXiv preprint arXiv:2001.04451},
  year={2020}
}

@article{choromanski2020rethinking,
  title={Rethinking attention with performers},
  author={Choromanski, Krzysztof and Likhosherstov, Valerii and Dohan, David and Song, Xingyou and Gane, Andreea and Sarlos, Tamas and Hawkins, Peter and Davis, Jared and Mohiuddin, Afroz and Kaiser, Lukasz and others},
  journal={arXiv preprint arXiv:2009.14794},
  year={2020}
}


@article{vig2019multiscale,
  title={A multiscale visualization of attention in the transformer model},
  author={Vig, Jesse},
  journal={arXiv preprint arXiv:1906.05714},
  year={2019}
}

@article{vig2019analyzing,
  title={Analyzing the Structure of Attention in a Transformer Language Model},
  author={Vig, Jesse and Yonatan, Belinkov},
  journal={arXiv preprint arXiv:1906.04284},
  year={2019}
}
